Quantile Rendering: Efficiently Embedding High-dimensional Feature on 3D Gaussian Splatting

Recent advancements in computer vision have successfully extended Open-vocabulary segmentation (OVS) to the 3D domain by leveraging 3D Gaussian Splatting (3D-GS). Despite this progress, efficiently rendering the high-dimensional features required for open-vocabulary queries poses a significant challenge. Existing methods employ codebooks or feature compression, causing information loss, thereby degrading segmentation quality. To address this limitation, we introduce Quantile Rendering (Q-Render), a novel rendering strategy for 3D Gaussians that efficiently handles high-dimensional features while maintaining high fidelity. Unlike conventional volume rendering, which densely samples all 3D Gaussians intersecting each ray, Q-Render sparsely samples only those with dominant influence along the ray. By integrating Q-Render into a generalizable 3D neural network, we also propose Gaussian Splatting Network (GS-Net), which predicts Gaussian features in a generalizable manner. Extensive experiments on ScanNet and LeRF demonstrate that our framework outperforms state-of-the-art methods, while enabling real-time rendering with an approximate ~43.7x speedup on 512-D feature maps. Code will be made publicly available.

==> table/ablation.Ksearch.tex <==
\begin{table*}[!tb]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|c|cc|cc|cc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Association}} & \multicolumn{1}{c|}{\multirow{2}{*}{$K$}} & \multicolumn{1}{c|}{\multirow{2}{*}{FPS}} & \multicolumn{2}{c|}{19 classes} & \multicolumn{2}{c|}{15 classes} & \multicolumn{2}{c}{10 classes} \\
     &  & & \mIoU & \mAcc & \mIoU & \mAcc & \mIoU & \mAcc \\
    \midrule

    V-Render~\citep{3dgs} & - & 19.92 & 27.86 & 39.52 & 30.01 & 43.36 & 42.47 & 57.45 \\
    \midrule

    \multirow{5}{*}{top-K~\citep{dr_splat}} & 5 & 23.75 & 26.69 & 36.86 & 28.97 & 41.27 & 40.49 & 54.83 \\
     & 10 & 21.16 & 26.62 & 38.49 & 28.63 & 42.28 & 39.92 & 56.38 \\
     & 20 & 14.71 & 26.59 & 36.52 & 29.34 & 41.35 & 40.85 & 54.97 \\
     & 40 & 6.82 & 26.71 & 38.70 & 28.63 & 42.15 & 39.87 & 55.58 \\
     & 80 & 2.59 & 26.79 & 36.60 & 29.73 & 41.83 & 41.11 & 55.41 \\
    \midrule

    \multirow{5}{*}{Q-Render (ours)} & 5 & 31.20 & 26.52 & 38.58 & 28.56 & 41.93 & 40.22 & 56.15 \\
     & 10 & 30.84 & 26.60 & 38.09 & 28.78 & 41.90 & 40.09 & 55.69 \\
     & 20 & 29.45 & 26.75 & 36.53 & 29.51 & 41.47 & 40.79 & 54.58 \\
     & 40 & 28.89 & 28.42 & 38.85 & 31.02 & 44.02 & 42.58 & 57.92 \\
     & 80 & 28.07 & 27.42 & 39.48 & 29.29 & 42.74 & 41.04 & 56.71 \\
    \bottomrule

    \end{tabular}}
    \caption{FPS and performance comparison by varying the number of Gaussians $K$.}
    \label{tab.Ksearch}
\end{table*}

==> table/ablation.feature_association.tex <==
\begin{table}[!t]
    \caption{
        Ablation study for the rendering algorithm variants.
    }
    \vspace{-3mm}
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|cc|cc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Association}} & \multicolumn{1}{c|}{\multirow{2}{*}{\Eqref{eq:volumetric rendering}}} & \multicolumn{2}{c|}{19 classes} & \multicolumn{2}{c}{15 classes} \\
    & & \mIoU & \mAcc & \mIoU & \mAcc \\
    \midrule
    
    V-Render~\citep{3dgs,langsplat} & \checkmark & 27.86 & \textbf{39.52} & 30.09 & 43.36 \\
    \midrule

    top-K & \checkmark & 26.71 & 38.70 & 28.63 & 42.15 \\
    3D-top-K~\citep{dr_splat} & & 22.44 & 31.40 & 26.31 & 38.03 \\
    3D-top-K-W & & 25.96 & 35.37 & 28.61 & 41.29 \\
    \midrule
    
    \samplernameshort (ours) & \checkmark & \textbf{28.42} & 38.85 & \textbf{31.02} & \textbf{44.02} \\
    3D-Quantile & & 15.74 & 23.47 & 18.70 & 31.30 \\
    3D-Quantile-W & & 25.26 & 34.22 & 28.01 & 38.68 \\
    \bottomrule
    \end{tabular}}
    \label{tab.feature_association}
\end{table}
